Fast and Blind Speech Copy-Move Detection and Localization in Noise

Copy-move forgery on speech (CMF), coupled with post-processing techniques, presents a great challenge to the forensic detection and localization of tampered areas. Most of the existing CMF detection approaches necessitate pre-segmentation of speech to facilitate similarity calculations among these segments. However, these approaches usually suffer from the problems of uncontrollable computational complexity and sensitivity to the presence of a word that is read multiple times within a speech recording. To address these issues, we propose a local feature tensors-based CMF detection algorithm that can transform duplicate detection and localization problems into a special tensor-matching procedure, accompanied by complete theoretical analysis as support. Through extensive experimentation, we have demonstrated that our method exhibits computational efficiency and robustness against post-processing techniques. Notably, it can effectively and blindly detect tampered segments, even those as short as a fractional second. These advantages highlight the promising potential of our approach for practical applications.

==> figures/subfigure.tex <==
\documentclass[smallextended]
\usepackage{lipsum}% Just for this example
\usepackage[dvipsnames]{xcolor}
\usepackage{tikz} 
\usepackage{amsmath,amsfonts}
\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{array}
%\usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
\usepackage{textcomp}
\usepackage{stfloats}
\usepackage{url}
\usepackage{verbatim}
\usepackage{graphicx}
\usepackage{cite}
\usepackage{pdfpages}
\hyphenation{op-tical net-works semi-conduc-tor IEEE-Xplore}
\usepackage{tikz,mathpazo}  
%\usepackage{subfigure}
%\usetikzlibrary{shapes.geometric, arrows,chains} 
\usetikzlibrary{shadows,arrows,positioning,shapes.geometric,chains} 
\usetikzlibrary{calc} 
\tikzstyle{straightline} = [line width = 1pt,-]

\usepackage{subfigure}
\begin{document}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=1.0\textwidth,height=0.3\textwidth]{txphotodongft.png} 
         \caption{$y=x$}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=1.0\textwidth,height=0.3\textwidth]{txphotodongft.png} 
         \caption{$y=3\sin x$}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=1.0\textwidth,height=0.3\textwidth]{txphotodongft.png} 
         \caption{$y=5/x$}
         \label{fig:five over x}
     \end{subfigure}
        \caption{Three simple graphs}
        \label{fig:three graphs}
\end{figure}

\end{document}
